FLAVR: Flow-Agnostic Video Representations for Fast Frame Interpolation

A majority of methods for video frame interpolation compute bidirectional optical flow between adjacent frames of a video, followed by a suitable warping algorithm to generate the output frames. However, approaches relying on optical flow often fail to model occlusions and complex non-linear motions directly from the video and introduce additional bottlenecks unsuitable for widespread deployment. We address these limitations with FLAVR, a flexible and efficient architecture that uses 3D space-time convolutions to enable end-to-end learning and inference for video frame interpolation. Our method efficiently learns to reason about non-linear motions, complex occlusions and temporal abstractions, resulting in improved performance on video interpolation, while requiring no additional inputs in the form of optical flow or depth maps. Due to its simplicity, FLAVR can deliver 3x faster inference speed compared to the current most accurate method on multi-frame interpolation without losing interpolation accuracy. In addition, we evaluate FLAVR on a wide range of challenging settings and consistently demonstrate superior qualitative and quantitative results compared with prior methods on various popular benchmarks including Vimeo-90K, UCF101, DAVIS, Adobe, and GoPro. Finally, we demonstrate that FLAVR for video frame interpolation can serve as a useful self-supervised pretext task for action recognition, optical flow estimation, and motion magnification.

==> scripts/qualitative_GoPro.tex <==
%% Qualitative Figures


\begin{figure*}[h]
    \centering
    \begin{subfigure}[b]{0.18\textwidth}
        \centering
        \includegraphics[width=\textwidth]{scripts/qualt_GoPro/im1_gt.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.18\textwidth}
        \centering
        \includegraphics[width=\textwidth]{scripts/qualt_GoPro/im1_qvi.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.18\textwidth}
        \centering
        \includegraphics[width=\textwidth]{scripts/qualt_GoPro/im1_FLAVR.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.18\textwidth}
        \centering
        \includegraphics[width=\textwidth]{scripts/qualt_GoPro/im1_qvi_err.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.18\textwidth}
        \centering
        \includegraphics[width=\textwidth]{scripts/qualt_GoPro/im1_flavr_err.pdf}
    \end{subfigure}
    
    %%%%%
    %%%%%
    
    \begin{subfigure}[b]{0.18\textwidth}
        \centering
        \includegraphics[width=\textwidth]{scripts/qualt_GoPro/im2_gt.png}
        \caption{GT Frame}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.18\textwidth}
        \centering
        \includegraphics[width=\textwidth]{scripts/qualt_GoPro/im2_qvi.png}
        \caption{Interpolated - QVI~\cite{xu2019quadratic}}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.18\textwidth}
        \centering
        \includegraphics[width=\textwidth]{scripts/qualt_GoPro/im2_flavr.png}
        \caption{Interpolated - FLAVR}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.18\textwidth}
        \centering
        \includegraphics[width=\textwidth]{scripts/qualt_GoPro/im2_qvi_err.png}
        \caption{Error Map, QVI}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.18\textwidth}
        \centering
        \includegraphics[width=\textwidth]{scripts/qualt_GoPro/im2_flavr_err.png}
        \caption{Error Map, FLAVR (Ours)}
    \end{subfigure}
    \vspace{-24pt}
    \caption{{\bf Qualitative comparison on GoPro dataset}. Error maps indicating the deviation from ground truth frame on GoPro dataset for QVI and \Ours{}. \Ours{} produces smoother predictions near motion boundaries and edges because of its more accurate frame interpolation.}
    \label{fig:qualt_figs_GoPro}
     \vspace{-24pt}
\end{figure*}

==> scripts/tables/Table_4x_Expmnts.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}
  \centering
  \small
%   \resizebox{0.45\textwidth}{!}{
  \begin{tabular}{@{} l *{5}{c} @{}} 
    \toprule  \\[-1em]
    && SuperSloMo~\cite{jiang2018super}  & DAIN~\cite{bao2019depth}  & QVI~\cite{xu2019quadratic} & \Ours \\
    \midrule
    PSNR && 30.8 & 32.49 & \underline{36.29} & {\bf 37.82} \\
    SSIM && 0.924 & 0.957 & \underline{0.980} & {\bf 0.983} \\
    \bottomrule 
  \end{tabular}
%   }
  \captionsetup{width=0.48\textwidth}
  \caption{{\bf Comparison with state-of-the-art methods for 4x interpolation} on Adobe dataset. FLAVR outperforms QVI by 1.6dB, DAIN by 5.3dB, and Super-SloMo by 7dB in PSNR.}
%   \label{tab:fourx_interpolation}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> scripts/tables/Table_8x_experiments.tex <==
%% Small intro to the results

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}
\parbox{.45\linewidth}{
  \centering
  \rowcolors{6}{gray!25}{white}
% \centering
% \small
  \begin{tabular}{@{} l *{6}{c} @{}} 
    \toprule  \\[-1em]
     \multirow{3}{*}{Method} &
     \multirow{3}{*}{Inputs} &
     \multicolumn{2}{c}{Adobe}  && \multicolumn{2}{c}{GoPro} \\
     \cmidrule{3-4} \cmidrule{6-7}
                                        &                   &   PSNR & SSIM &&  PSNR & SSIM \\
    \midrule
    DAIN~\cite{bao2019depth}            &   RGB+Depth+Flow  &  29.50&0.910  && 29&0.91    \\
    QVI~\cite{xu2019quadratic}          &   RGB+Flow        &  \textbf{33.68}&\textbf{0.97 } && \underline{30.55} & \underline{0.933}     \\
    \midrule
    \midrule
    DVF~\cite{liu2017video}             &   RGB             &  28.23 & 0.896 && 21.94&0.776      \\
    SuperSloMo~\cite{jiang2018super}    &   RGB             &  30.66 & 0.391 && 28.52&0.891     \\
    \Ours{}                           &   RGB             &   \underline{32.20} & \underline{0.957}     && {\bf 31.31}& {\bf 0.94}    \\
    \bottomrule 
  \end{tabular}}
  \captionsetup{width=0.45\textwidth}
  \caption{{\bf Comparison with state-of-the-art methods for 8x interpolation} on Adobe and GoPro datasets. FLAVR outperforms all previous work that use only RGB as input. Overall, FLAVR achieves the best performance on GoPro and the second best on Adobe.}
  \label{tab:eightx_interpolation}
}
%
%
\parbox{.45\linewidth}{
  \centering
    \begin{tabular}{@{} l *{5}{c} @{}} 
    \toprule  \\[-1em]
    && SuperSloMo~\cite{jiang2018super}  & DAIN~\cite{bao2019depth}  & QVI~\cite{xu2019quadratic} & \Ours \\
    \midrule
    PSNR && 30.8 & 32.49 & \underline{36.29} & {\bf 37.82} \\
    SSIM && 0.924 & 0.957 & \underline{0.980} & {\bf 0.983} \\
    \bottomrule 
  \end{tabular}
%   }
  \captionsetup{width=0.48\textwidth}
  \caption{{\bf Comparison with state-of-the-art methods for 4x interpolation} on Adobe dataset. FLAVR outperforms QVI by 1.6dB, DAIN by 5.3dB, and Super-SloMo by 7dB in PSNR.}
  \label{tab:fourx_interpolation}
  }
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> scripts/tables/actionTable.tex <==
\begin{wraptable}{r}{3.5cm}
%\centering
    %\captionsetup{width=.4\textwidth}
    \caption{{\bf FLAVR for action recognition}. Results of using FLAVR as a self-supervised pretext task for action recognition on UCF101 and HMDB51. 
    %  The upper table includes the baselines and the state-of-the-art contrastive-based self-supervised learning method, DPC~\cite{han2019video}. The lower table presents self-supervised approaches with pixel-level pretext tasks. 
    %  FLAVR significantly outperforms the training from scratch baseline and other self-supervised approaches that use pixel-level pretext tasks.
    }
    \label{tab:actionUCF}
    %\resizebox{0.4\textwidth}{!}{
    % \centering
    {\small
    \begin{tabular}{l c c c c}
        \toprule
        Method & pretrained & Arch. & UCF101 & HMDB51 \\
        %\midrule
        %\midrule
        Random Init.                                & -         & R3D-18                & 50.02 &      19.00  \\
        Supervised & Kinetics-400                           &       R3D-18             &   87.70   &      59.10 \\
        Contrastive~\cite{han2019video} & Kinetics-400              & R3D-18              &   68.20   &      34.50  \\
        %\midrule
        Video-GAN~\cite{vondrick2016generating} & UCF101    &     Custom          & 52.10 &      -   \\
        LMD\cite{luo2017unsupervised}           & NTU RGB   &     Custom         & 53.00 &      - \\
        DVF \cite{liu2017video} &  UCF101                   &   Custom            & 52.40 &      - \\
        \Ours{} & Vimeo-90K                           &      R3D-18          & 63.10 &      23.48 \\
        \bottomrule
    \end{tabular}}
\end{wraptable}

==> scripts/tables/flowtable.tex <==
\begin{wraptable}{r}{0.4\textwidth}%\[!htb\]
  \captionsetup{width=0.4\textwidth}
     \caption{{\bf FLAVR for optical flow estimation}. Comparison between FLAVR and other approaches for optical flow prediction on MPI Sintel~\cite{Butler_ECCV_2012} and Kitti datasets~\cite{Menze2015CVPR}.}
    \label{tab:SSL_flow}
    \resizebox{0.4\textwidth}{!}{
    \begin{tabular}{l c c c c}
        \toprule
         & FlowNet2.0~\cite{ilg2017flownet} & Random Init. & Finetune on \Ours{} \\
        \midrule
        MPI-Clean~\cite{Butler_ECCV_2012} & 2.02 & 4.41 & 2.92 \\
        MPI-Final~\cite{Butler_ECCV_2012} & 3.14 & 5.27 & 3.90 \\
        Kitti-12~\cite{Geiger2012CVPR} & 4.09 & 9.25  & 5.23 \\
        Kitti-15~\cite{Menze2015CVPR} & 10.06 & 17.22 & 13.68 \\
        \bottomrule
    \end{tabular}}
\end{wraptable}

==> scripts/tables/lowfpsTracking.tex <==
\begin{wraptable}{r}{0.3\textwidth}
  \centering
  \captionsetup{width=0.3\textwidth}
  \caption{{\bf Enhancing video object segmentation on DAVIS dataset using FLAVR}. Comparison against CRW~\cite{jabri2020space}.
}
  \label{tab:tracking}
  \resizebox{0.3\textwidth}{!}{
% \centering
% \small
\begin{tabular}{@{} l *{4}{c} @{}}
\toprule
\midrule
& \multicolumn{3}{c}{\textbf{15 $\rightarrow$ 30 FPS}} \\
 \cline{2-4}
&   $\mathcal{J}\&\mathcal{F}_{\text{m}}$ & $\mathcal{J}_{\text{m}}$ & $\mathcal{F}_{\text{m}}$ \\
CRW & 65.5 & 62.8 & 68.2 \\
FLAVR+CRW & \textbf{66.6} & \textbf{63.9} & \textbf{69.4} \\
& \multicolumn{3}{c}{\textbf{8 $\rightarrow$ 30 FPS}} \\
 \cline{2-4}
CRW & 65.5 & 62.8 & 68.2 \\
FLAVR+CRW & \textbf{66.6} & \textbf{63.9} & \textbf{69.4} \\
\bottomrule
\end{tabular}}
% \vspace{-8pt}
%   \vspace{-8pt}
\end{wraptable}
